Legion: Best-First Concolic Testing

Concolic execution and fuzzing are two complementary coverage-based testing techniques. How to achieve the best of both remains an open challenge. To address this research problem, we propose and evaluate Legion. Legion re-engineers the Monte Carlo tree search (MCTS) framework from the AI literature to treat automated test generation as a problem of sequential decision-making under uncertainty. Its best-first search strategy provides a principled way to learn the most promising program states to investigate at each search iteration, based on observed rewards from previous iterations. Legion incorporates a form of directed fuzzing that we call approximate path-preserving fuzzing (APPFuzzing) to investigate program states selected by MCTS. APPFuzzing serves as the Monte Carlo simulation technique and is implemented by extending prior work on constrained sampling. We evaluate Legion against competitors on 2531 benchmarks from the coverage category of Test-Comp 2020, as well as measuring its sensitivity to hyperparameters, demonstrating its effectiveness on a wide variety of input programs.

==> Figures/MCTS-guidedFuzzingInLegion.tex <==
\begin {tikzpicture}[
  transform canvas={scale=1.9},
  yshift=10, xshift=4,
  auto, node distance =0.8cm and 0.8cm, on grid, semithick,
  state/.style = {circle, top color=white, bottom color=white, 
                  draw, black, text=black, line width=0.1mm,
                  , scale=0.1mm},
  corner/.style = {rectangle, top color=white, bottom color=white, 
                  draw, white, text=black, scale=0.5},
]

\draw[pattern=north east lines, pattern color=black, line width=0.1mm] (1.2,0) -- (1.6, 0.692) -- (2, 0);

\node[state]  (Entry) at (1, 1.73) {};
\node[corner] (EntryNote) [right  = 1.3 of Entry] {~Program entry state};
\path[->, dashed, line width=0.1mm] (Entry) edge [] (EntryNote);

\node[state] (Fuzzing) [below right = 0.693 and 0.4 of Entry] {};
\node[corner] (FuzzingNote) [right  = 1.1 of Fuzzing] {\begin{tabular}{l} Program path \\ selected for fuzzing\end{tabular}};
\path[->, dashed, line width=0.1mm] (Fuzzing) edge [] (FuzzingNote);

\node[state] (Dashed) [below right = 1.038 and 0.6 of Entry] {};
\node[state] (Node5) [below right = 1.038 and 0.2 of Entry] {};

\node[state] (Node1) [below left = 0.693 and 0.4 of Entry] {};
\node[state] (Node2) [below left = 1.039 and 0.6 of Entry] {};
\node[state] (Node3) [below left = 1.039 and 0.2 of Entry] {};
\node[corner, scale=1, fill=transparent] (Node4) [below = 0.7 of Node1] {\begin{tabular}{c} ... \\ ...... \end{tabular}};

\coordinate  (Uncovered) at (1.6, 0.481);
\node[corner] (UncoveredNote) [right = 0.31 of Uncovered]
{\begin{tabular}{l}Unknown paths\end{tabular}};
\path[->, dashed, line width=0.1mm] (Uncovered) edge [] (UncoveredNote);

\coordinate  (Covered) at (1.2, 0.225);
\node[corner] (CoveredNote) [right  = 0.9 of Covered] {Observed paths};
\path[->, dashed, line width=0.1mm] (Covered) edge [] (CoveredNote);

\node[corner, scale=1] (Node6) [below right = 0.3 and 0.05 of Node5] {...};
\node[corner, scale=1] (Node7) [below left = 0.6 and 0.1 of Node5] {...};

\draw [decorate,decoration={brace,amplitude=3pt,mirror,raise=0pt},yshift=-1pt, line width=0.1mm] 
(0.801,0) -- (2, 0) node [black,midway,xshift=0pt, yshift=-10pt, scale=0.475] {Score: estimate the likelihood of finding new paths};

\draw [decorate,decoration={brace,amplitude=3pt,mirror,raise=0pt}, xshift=-3pt, yshift=0pt, line width=0.1mm] 
(1, 1.73) -- (0, 0) node [black,midway,xshift=-21pt, yshift=-19pt, scale=0.475, rotate=60] {A concrete execution trace};

\draw[line width=0.1mm, dashed] (0,0) -- (Node2);
\draw[line width=0.1mm] (Node1) -- (Node2);
\draw[line width=0.1mm] (Node1) -- (Node3);
\draw[line width=0.1mm, dashed] (Node4) -- (Node2);
\draw[line width=0.1mm, dashed] (Node4) -- (Node3);

\draw[line width=0.1mm] (Node1) -- (Entry) -- (Fuzzing);
\draw[line width=0.1mm] (0.801,0) -- (Node5) -- (Fuzzing) -- (Dashed);
\draw[line width=0.1mm] (1.2,0) -- (Dashed) -- (2, 0);

\end{tikzpicture}


==> Makefile <==
.PHONY: pdf

all: Legion-ASE.pdf

LATEX ?= pdflatex -interaction=nonstopmode

OtherTexs=$(wildcard Sections/*.tex Figures/*.tex Tables/*.tex)
OtherTemplates=$(wildcard *.bst *.cls)

Legion-ASE.pdf: Legion-ASE.tex Legion-ASE.bib $(OtherTexs) $(OtherTemplates)
	@echo "latex first pass..."
	@((${LATEX} $< > .log); \
	if [ $$? -ne 0 ]; then \
            echo "latex failed. Output follows: "; cat .log; \
            exit 1; \
        fi)
	@echo "bibtex...";
	@bibtex ${<:%.tex=%} > .log
	@echo "latex second pass...";
	@${LATEX} $< > .log
	@while ( grep -q 'may have changed' $*.log) \
	do echo "latex nth pass..."; ${LATEX} $< > .log; done
	@grep -i 'undefined' .log > .undef; \
	if [ ! -z "$$(cat .undef)" ]; then \
            echo "Undefined references: "; cat .undef; \
        fi


clean:
	-rm -f Legion-ASE.aux Legion-ASE.log Legion-ASE.out
	-rm -f Legion-ASE.blg Legion-ASE.bbl
	-rm -f Legion-ASE.fdb_latexmk Legion-ASE.fls Legion-ASE.synctex.gz


==> Sections/FutureWork.tex <==
\section{Future Work} \label{sec: future work}

We believe \Legion's greatest value lies in its future potential.
First, we intend to apply it to examine the effectiveness of different
score functions, to represent different reward heuristics.
This paper proposes a simple score function in \cref{sec: a reward evaluation heuristic} and we briefly compared it against random selection in
\cref{sec: sensitivity experiment results} as an example. 
Its modular design enables adding broader information into the score function in future, including the potential for contextual score functions.

We also intend to extend \Legion so that it can also incorporate other
input generation techniques and learn which technique is best to use for
different parts of the program: both in terms of their performance and
accuracy.

We also intend to investigate extending \Legion's MCTS, by adopting ideas~\cite{levine2017rotting}
that allow a node's rewards to be reduced over time, reflecting the assumption that that the more we have simulated from a node, the fewer
new paths there remain to be discovered from it. The score of each node may also be affected by its type or other contextual features~\cite{ContextualBandit}.

\iffalse % Toby: cut this since I dont' understand it
\Legion can also be used on transfer learning. Exploration settings preferable for one program structure give us insight how on to design a setting that works well on others, but how to summarise and transfer this knowledge remains unknown. \Legion models them as hyperparameters and evaluated their effectiveness in \cref{sec: sensitivity experiment results}. \Legion also attempted to transfer the knowledge on one benchmark suite to all suites from the competition. 
\fi




% \subsubsection{Code coverage.} Measuring the percentage of code coverage over time in the program under test is a simple but effective way to evaluate the efficiency of a program exploration strategy. Well-established tools like \texttt{Gcov} are often used in the field {\color{green} cite which paper used it} to measure the line coverage. Our implementation works as follows:

% \begin{itemize}
%   \item Legion selects a node to fuzz in the selection step
%   \item Legion generates a bunch of inputs and executes them on the instrumented binary
%   \item Legion executes each of the inputs on the original binary. After each binary execution, it also invokes \texttt{Gcov} to obtain and record the new coverage score. The increment of the current score over the previous is treated as the reward of that simulation.
%   \item Legion integrates the execution traces from instrumented binary execution to the tree.
%   \item Legion propagates the reward to each node selected by the selection step.
% \end{itemize}

% $$\bar{X_i} = \sum{coverage} / N_{\text{sel}}(i)$$


% \subsubsection{Time consumption} In addition to the number of invocations of APPFuzzing, the time consumption of each APPFuzzing (more specifically, each constraint solving) is also crucial to the overall efficiency. Consider the situation of comparing the simulation node of the parent with its children to balances the following trade-off: 

% \begin{itemize}
%   \item {\color{blue} Parent nodes are empirically fuzzed more than each of their children (need to explain?). Due to APPFuzzing's increasing marginal returns from constraint solving, with one constraint solving, more inputs can be generated from the parent than one of its children}.
%   \item The parents have less constraints than their children, therefore solving their constraints tend to take less time in general.
%   \item The paths found by fuzzing the parents will more likely to spread over all children while fuzzing on a specific child tend to limit the findings to its own subtree.
%   \item On the other hand, if the constraint of a child with a large subtree turns out to block most inputs, then it is better to fuzz on that child directly instead. Hence spending more time to generate less inputs from the child may turn out to be more beneficial. 
% \end{itemize}
 
% \textsc{Legion} aims to balance these trade-offs by taking time consumption on APPFuzzing solving as a penalisation. The first part of the UCT function aims to estimate the future reward with the past average. However, it is not accurate in this case, as the estimated number of new inputs from each APPFuzzing call doubles every time. We adjust this with a coefficient that optimistically estimates the next number of inputs can be generated.

% $$\bar{X_i} = - C_T * \frac{\sum{T_i}}{N_{\text{sel}}(i)} * \frac{1}{2^{N_{\text{sel}}(i)}} $$

% where the constant $C_T$ is used to controls the sensitivity to time, and adjust the time penalisation if it is too high/low to affect others in various programs, $T_i$ is the amount of time spent on APPFuzzing that node.

% These function can be further composited.

% 1. The score function can use the result of vulnerability detectors as a reward. It subjects to the problem of MCTS assumes the solution is not rare to find, while vulnerabilities are rare.

% 2. This can further be expanded to allow Legion to choose from multiple APPFuzzing tools as arms and apply the one with highest empirical performance on different programs or program locations. This extension requires Legion to choose the most suitable tool to fuzz the most rewarding node. Hence the score of each node comes from two aspects, the accuracy of the tool to preserve the path to the node, and the availability to find new paths beneath the node. The current setting has the data needed for this extension: the relation between $N_{exc}$ and $N_{\text{sel}}(i)$ indicates the accuracy, while the existence of new paths under the node can be inferred from the relation between $N_{new}$ and $N_{exc}$.

% {\color{blue}
%   3. Furthermore, Legion can demonstrate the accuracy and performance of various APPFuzzing tools as a framework.
% }

% 3. Instead of applying the vanilla MAB algorithm on each node, a variation named rotting bandits might be more suitable to software testing. Rotting bandits reduces the rewards of an arm over time, which aligns to the fact that the more we have simulated from a node with a tool, the less chance the tool can find new paths from the node because of either the less untested space there will be under the node or the non-uniform limitation of tool tends to only find paths of certain property.



% 4. In addition, the ratio of $N_{exc} / N_{\text{sel}}(i)$ can be used to measure the accuracy of the APPFuzzing tool utilised. Section \label{sec: Future Work} discusses this in detail.


==> TODO <==
# Turn the [  ] into [ X ] when each is done

[x] Check for remaining \ref{...} (these should all be \cref{...})
[x] Check for APPFuzz, APPFuzzing etc. These should all use the \APPF macro
[x] Check for any uses of Legion. These sould all use the \Legion macro
[x] Check for any uses of angr. These should all use the \Angr macro.
[x] Check for consistency of naming and font for QuickSampler
[x] Check all remaining FIXMEs
[x] Check for remaining coloured text
[x] Spellcheck for Related work, Future work, and conclusion
[x] Update abstract on submission site
[ ] Check references: capitalisation, consistency of conference names, etc.
[x] If we decided to use the competition result (because we cannot fix the low score in the new results), we need to specify Legion used 8 cores (instead of 2) in the Experiment section

If time:
[x]  rename red/white/black/purple/golden nodes to
            concolic/concrete/redundant/symbolic/simulation



==> Tables/AlternativeSensitivityResult.tex <==
\begin{tabular}{|r|l|l|}
    \hline
    Settings & Baseline & Setting 2 \\
    \hline\hline
    Overall score & 7509.79 & 8124.6 \\
    \hline
    p-value & - & 0.005983 \\
    \hline
\end{tabular}

==> Tables/CompetitionResult2.tex <==

\begin{tabular}{|r|lllllllll|}
    \hline
    Participants & \Legion{\color{red}*} & \texttt{KLEE}~\cite{cadar2008klee} & \texttt{CoVeriTest}~\cite{beyer2019coveritest} & \texttt{HybridTiger}~\cite{ruland2020hybridtiger} & \texttt{LibKluzzer}~\cite{le2020llvm} & \texttt{PRTest} & \texttt{Symbiotic}~\cite{Symbiotic7} & \texttt{Tracer-X}~\cite{jaffar2020tracerx}  & \texttt{VeriFuzz}~\cite{VeriFuzz} \\
    \hline\hline
    % {\color{red} Normailised Average**} & $1455.908002$ & $1515.97673$ & $1588.862835$ & $1541.850942$ & $1759.050529$ & $584.57209$ & $969.1994602$ & $1382.674571$ & $1746.261043$ \\
    % \hline
    {\color{red} Normailised Average***} & $1502.984227$ & $1492.940073$ & $1555.807154$ & $1504.493807$ & $1742.850222$ & $630.8958136$ & $1036.312556$ & $1346.157462$ & $1734.025271$ \\
    \hline
    % {\color{red} Normailised Average****} & $1452.564362$ & $1443.719195$ & $1504.030926$ & $1454.700936$ & $1688.051552$ & $610.038214$ & $997.2578185$ & $1299.7722$ & $1678.917913$ \\
    % \hline
\end{tabular}




==> Tables/SensitivityResult.tex <==
% \begin{tabular}{|r|lllll|}
%     \hline
%     Settings & Overall score & t-Test \\
%     \hline\hline
%     Baseline &  $\frac{1}{\sqrt{2}}$ & UCT &  $\infty$ &  $\infty$ & 3 \\
%     \hline
%     Setting 1 & 0 & UCT &  $\infty$ &  $\infty$ & 3 \\
%     \hline
%     Setting 2 & 100 & UCT &  $\infty$ &  $\infty$ & 3 \\
%     \hline
%     Setting 3 &  $\frac{1}{\sqrt{2}}$ & Random &  $\infty$ &  $\infty$ & 3 \\
%     \hline
%     Setting 4 &  $\frac{1}{\sqrt{2}}$ & UCT & 1 &  $\infty$ & 3 \\
%     \hline
%     Setting 5 &  $\frac{1}{\sqrt{2}}$ & UCT &  $\infty$ & 1 & 3 \\
%     \hline
%     Setting 6 &  $\frac{1}{\sqrt{2}}$ & UCT &  $\infty$ &  $\infty$ & 1 \\
%     \hline
%     Setting 7 &  $\frac{1}{\sqrt{2}}$ & UCT &  $\infty$ &  $\infty$ & 5 \\
%     \hline
% \end{tabular}

\begin{tabular}{|r|l|l|l|l|l|l|l|l|l|}
    \hline
    Settings & Baseline & Setting 1 & Setting 2 & Setting 3 & Setting 4  & Setting 5 & Setting 6 & Setting 7 & Setting 8\\
    \hline\hline
    Overall score & 4960.18 & 5320.41 & 5340.86 & 4679.28 & 4785.44 & 4701.77 & 5018.03 & 5104.16 & 4929.94 \\
    \hline
    p-value & - & 0.030585959 & 0.0230889 & 4.81237E-06 & 9.6681E-10 & 3.4225E-07 & 0.024712147 & 0.119176209 & 0.068142969\\
    \hline
\end{tabular}

==> Tables/ThirdSensitivityResult.tex <==
\begin{tabular}{|r|l|l|}
    \hline
    Settings & Baseline & Setting 2 \\
    \hline\hline
    Overall score & 2243.02 & 3169.42 \\
    \hline
    p-value & - & 5.80334E-07 \\
    \hline
\end{tabular}
